Encoded Value-at-Risk: A Predictive Machine for Financial Risk Management

Measuring risk is at the center of modern financial risk management. As the world economy is becoming more complex and standard modeling assumptions are violated, the advanced artificial intelligence solutions may provide the right tools to analyze the global market. In this paper, we provide a novel approach for measuring market risk called Encoded Value-at-Risk (Encoded VaR), which is based on a type of artificial neural network, called Variational Auto-encoders (VAEs). Encoded VaR is a generative model which can be used to reproduce market scenarios from a range of historical cross-sectional stock returns, while increasing the signal-to-noise ratio present in the financial data, and learning the dependency structure of the market without any assumptions about the joint distribution of stock returns. We compare Encoded VaR out-of-sample results with eleven other methods and show that it is competitive to many other well-known VaR algorithms presented in the literature.

==> tabs/loss_table_FSE_1.tex <==
\toprule
& \textbf{Sener} & \textbf{Lopez} & \textbf{Sarma} & \textbf{Quadratic} & \textbf{Caporin 1} & \textbf{Caporin 2} & \textbf{Caporin 3} & \textbf{Quantile } \\
\midrule

\textbf{RiskMetrics} & 0.0192(10) & 0.0269(10) & 0.047(10) & 0.0003(10) & 2.9136(10) & 0.0156(10) & 0.0531(10) & 0.0336(9) \\
\textbf{Variance - Covariance} & 0.0188(8) & 0.0286(11) & 0.0486(12) & 0.0004(11) & 3.5275(11) & 0.0237(11) & 0.0612(11) & 0.0299(7) \\
\textbf{Historical} & 0.027(12) & 0(1)  & 0.0342(6) & 0(1)  & 0(1)  & 0(1)  & 0(1)  & 0.0792(12) \\
\textbf{Filtered Historical} & 0.0165(3) & 0.0101(6) & 0.0335(5) & 0.0001(4) & 1.0394(6) & 0.0057(5) & 0.0188(6) & 0.0452(11) \\
\textbf{Monte Carlo} & 0.0189(9) & 0.0286(11) & 0.0484(11) & 0.0004(12) & 3.8677(12) & 0.0261(12) & 0.0662(12) & 0.0304(8) \\
\textbf{GARCH} & 0.0158(2) & 0.0236(8) & 0.0439(8) & 0.0003(9) & 2.2573(9) & 0.0147(8) & 0.0433(9) & 0.0298(6) \\
\textbf{E-GARCH} & 0.0154(1) & 0.0236(8) & 0.0442(9) & 0.0003(8) & 2.2136(8) & 0.015(9) & 0.0416(8) & 0.0284(3) \\
\textbf{CAViaR Symmetric} & 0.0175(6) & 0.0067(3) & 0.0313(2) & 0.0001(3) & 0.7565(3) & 0.0052(4) & 0.0161(3) & 0.0342(10) \\
\textbf{CAViaR Asymmetric} & 0.0176(7) & 0.0067(3) & 0.0314(3) & 0.0001(6) & 0.8501(5) & 0.0081(7) & 0.0163(4) & 0.0294(4) \\
\textbf{CAViaR Garch} & 0.0169(4) & 0.0084(5) & 0.0323(4) & 0.0001(5) & 0.7833(4) & 0.0051(3) & 0.0178(5) & 0.0296(5) \\
\textbf{CAViaR Adaptive} & 0.021(11) & 0.0152(7) & 0.0419(7) & 0.0002(7) & 1.1376(7) & 0.0069(6) & 0.0261(7) & 0.0227(1) \\
\textbf{Encoded VaR} & 0.0171(5) & 0.0044(2) & 0.0287(1) & 0(2)  & 0.2719(2) & 0.001(2) & 0.0071(2) & 0.0271(2) \\
\bottomrule

==> tabs/loss_table_FSE_5.tex <==

\begin{table*}[pos=t]
  \centering
  \caption{1-day 95\% VaR Losses(with their rank): FSE portfolio}
    \begin{tabular}{lllllllll}
    \toprule
          & \textbf{Sener} & \textbf{Lopez} & \textbf{Sarma} & \textbf{Quadratic} & \textbf{Caporin 1} & \textbf{Caporin 2} & \textbf{Caporin 3} & \textbf{Quantile } \\
    \midrule
    \textbf{RiskMetrics} & 0.1093(11) & 0.0926(12) & 0.1059(12) & 0.0018(9) & 18.3029(10) & 0.129(9) & 0.2421(11) & 0.0209(10) \\
    \textbf{Variance - Covariance} & 0.095(7) & 0.0774(6) & 0.091(6) & 0.0019(10) & 17.9546(9) & 0.1441(10) & 0.2343(9) & 0.0193(7) \\
    \textbf{Historical} & 0.0919(6) & 0.0286(1) & 0.0499(1) & 0.0007(2) & 6.4162(2) & 0.0493(1) & 0.0929(2) & 0.0181(4) \\
    \textbf{Filtered Historical} & 0.0918(5) & 0.0842(9) & 0.0983(9) & 0.0013(6) & 16.1516(6) & 0.1(6) & 0.197(6) & 0.0262(12) \\
    \textbf{Monte Carlo} & 0.0972(8) & 0.0791(7) & 0.0926(7) & 0.0019(11) & 18.4593(11) & 0.1484(11) & 0.24(10) & 0.0193(8) \\
    \textbf{GARCH} & 0.0994(10) & 0.0892(11) & 0.1025(11) & 0.0017(8) & 16.8352(8) & 0.1207(8) & 0.2267(8) & 0.0198(9) \\
    \textbf{E-GARCH} & 0.0979(9) & 0.0875(10) & 0.101(10) & 0.0016(7) & 16.2579(7) & 0.1179(7) & 0.2214(7) & 0.019(6) \\
    \textbf{CAViaR Symmetric} & 0.0737(3) & 0.0606(3) & 0.0764(3) & 0.001(5) & 9.3152(4) & 0.0656(5) & 0.1419(4) & 0.017(3) \\
    \textbf{CAViaR Asymmetric} & 0.0599(1) & 0.0471(2) & 0.0634(2) & 0.0006(1) & 5.918(1) & 0.0493(2) & 0.0839(1) & 0.0233(11) \\
    \textbf{CAViaR Garch} & 0.0763(4) & 0.0673(5) & 0.0828(5) & 0.001(4) & 9.6626(5) & 0.0619(4) & 0.1469(5) & 0.0189(5) \\
    \textbf{CAViaR Adaptive} & 0.1239(12) & 0.0808(8) & 0.0949(8) & 0.0022(12) & 18.5313(12) & 0.1663(12) & 0.2535(12) & 0.0153(1) \\
    \textbf{Encoded VaR} & 0.0636(2) & 0.064(4) & 0.0785(4) & 0.0009(3) & 8.6775(3) & 0.0551(3) & 0.1322(3) & 0.0165(2) \\
    \bottomrule
    \end{tabular}
  \label{tab:addlabel}
\end{table*}



==> tabs/loss_table_LSE_1.tex <==
& \textbf{Sener} & \textbf{Lopez} & \textbf{Sarma} & \textbf{Quadratic} & \textbf{Caporin 1} & \textbf{Caporin 2} & \textbf{Caporin 3} & \textbf{Quantile } \\
\midrule
\textbf{RiskMetrics} & 0.0187(9) & 0.0287(10) & 0.042(11) & 0.0006(10) & 6.8512(12) & 0.0517(10) & 0.0783(12) & 0.03(7) \\
\textbf{Variance - Covariance} & 0.0196(10) & 0.027(9) & 0.0404(9) & 0.0006(11) & 6.2452(10) & 0.0529(11) & 0.0752(10) & 0.0232(5) \\
\textbf{Historical} & 0.0208(12) & 0.0017(1) & 0.0274(6) & 0(1)  & 0.263(1) & 0.0013(1) & 0.0051(1) & 0.0471(12) \\
\textbf{Filtered Historical} & 0.0155(8) & 0.0287(10) & 0.0424(12) & 0.0004(9) & 6.0327(9) & 0.0315(9) & 0.0646(9) & 0.0399(11) \\
\textbf{Monte Carlo} & 0.0202(11) & 0.0287(10) & 0.0419(10) & 0.0007(12) & 6.4679(11) & 0.0545(12) & 0.0772(11) & 0.0235(6) \\
\textbf{GARCH} & 0.0121(2) & 0.0101(6) & 0.0263(4) & 0.0003(7) & 2.214(7) & 0.0188(7) & 0.0314(6) & 0.0149(2) \\
\textbf{E-GARCH} & 0.0119(1) & 0.0152(8) & 0.0302(8) & 0.0004(8) & 3.5045(8) & 0.028(8) & 0.0477(8) & 0.0203(4) \\
\textbf{CAViaR Symmetric} & 0.0132(5) & 0.0084(5) & 0.0265(5) & 0.0001(4) & 1.1399(5) & 0.0079(4) & 0.0172(5) & 0.0331(8) \\
\textbf{CAViaR Asymmetric} & 0.0124(3) & 0.0034(2) & 0.0205(1) & 0.0001(5) & 0.9043(4) & 0.0089(5) & 0.0135(3) & 0.0335(9) \\
\textbf{CAViaR Garch} & 0.0131(4) & 0.0068(4) & 0.0247(3) & 0.0001(3) & 0.8822(3) & 0.0059(3) & 0.0142(4) & 0.0395(10) \\
\textbf{CAViaR Adaptive} & 0.015(7) & 0.0101(6) & 0.0293(7) & 0.0002(6) & 2.1521(6) & 0.0148(6) & 0.0343(7) & 0.0112(1) \\
\textbf{Encoded VaR} & 0.0141(6) & 0.0055(3) & 0.0241(2) & 0(2)  & 0.432(2) & 0.002(2) & 0.0086(2) & 0.0168(3) \\

==> tabs/loss_table_LSE_5.tex <==
\begin{table*}[width=2.0\linewidth,cols=9,pos=t!]
  \centering
  \caption{1-day 95\% VaR Losses(with their rank): LSE portfolio}
  \begin{tabular*}{\tblwidth}{@{}LCCLCCLCC@{}}
\toprule
          & \textbf{Sener} & \textbf{Lopez} & \textbf{Sarma} & \textbf{Quadratic} & \textbf{Caporin 1} & \textbf{Caporin 2} & \textbf{Caporin 3} & \textbf{Quantile } \\
    \midrule
    \textbf{RiskMetrics} & 0.0735(10) & 0.0676(11) & 0.0766(11) & 0.0014(10) & 20.4812(11) & 0.1687(11) & 0.1654(11) & 0.0082(8) \\
    \textbf{Variance - Covariance} & 0.0688(8) & 0.0591(8) & 0.0683(8) & 0.0014(8) & 18.5117(9) & 0.1626(9) & 0.1595(9) & 0.0059(3) \\
    \textbf{Historical} & 0.0527(5) & 0.022(1) & 0.0353(1) & 0.0006(3) & 5.3195(1) & 0.0438(3) & 0.0695(2) & 0.0126(11) \\
    \textbf{Filtered Historical} & 0.0938(12) & 0.0946(12) & 0.1023(12) & 0.0016(12) & 32.6918(12) & 0.2147(12) & 0.2111(12) & 0.0112(9) \\
    \textbf{Monte Carlo} & 0.0691(9) & 0.0608(9) & 0.0699(9) & 0.0014(9) & 18.6848(10) & 0.1627(10) & 0.161(10) & 0.0059(2) \\
    \textbf{GARCH} & 0.0532(6) & 0.0405(3) & 0.0515(3) & 0.0008(6) & 9.2008(6) & 0.0762(6) & 0.0979(6) & 0.0068(5) \\
    \textbf{E-GARCH} & 0.0609(7) & 0.0473(7) & 0.0574(7) & 0.0011(7) & 12.9884(7) & 0.1077(7) & 0.123(7) & 0.0073(6) \\
    \textbf{CAViaR Symmetric} & 0.0511(4) & 0.0456(6) & 0.0564(6) & 0.0007(4) & 8.599(4) & 0.0636(4) & 0.0878(4) & 0.0119(10) \\
    \textbf{CAViaR Asymmetric} & 0.0418(2) & 0.0422(4) & 0.0528(5) & 0.0004(1) & 6.656(3) & 0.0414(1) & 0.0672(1) & 0.0137(12) \\
    \textbf{CAViaR Garch} & 0.0477(3) & 0.0422(5) & 0.0527(4) & 0.0007(5) & 8.8427(5) & 0.0673(5) & 0.0965(5) & 0.0081(7) \\
    \textbf{CAViaR Adaptive} & 0.0744(11) & 0.0608(9) & 0.0701(10) & 0.0015(11) & 17.1183(8) & 0.1585(8) & 0.1584(8) & 0.0024(1) \\
    \textbf{Encoded VaR} & 0.0413(1) & 0.0372(2) & 0.0479(2) & 0.0005(2) & 6.1678(2) & 0.0431(2) & 0.0742(3) & 0.0065(4) \\
    \bottomrule
    \end{tabular*}%
  \label{tab:addlabel}%
\end{table*}%


==> tabs/loss_table_SP_1.tex <==
      & \textbf{Sener} & \textbf{Lopez} & \textbf{Sarma} & \textbf{Quadratic} & \textbf{Caporin 1} & \textbf{Caporin 2} & \textbf{Caporin 3} & \textbf{Quantile } \\
\midrule
\textbf{RiskMetrics} & 0.0169(5) & 0.0149(8) & 0.0311(6) & 0.0013(10) & 6.2761(10) & 0.0901(10) & 0.0865(10) & 0.0962(11) \\
\textbf{Variance - Covariance} & 0.0264(12) & 0.0215(11) & 0.038(12) & 0.0018(11) & 9.3167(11) & 0.1524(11) & 0.1098(11) & 0.0893(9) \\
\textbf{Historical} & 0.022(9) & 0.0099(5) & 0.0333(10) & 0.0008(6) & 2.7744(6) & 0.0365(4) & 0.0574(6) & 0.0106(1) \\
\textbf{Filtered Historical} & 0.0146(3) & 0.0116(7) & 0.0302(3) & 0.001(9) & 4.4435(8) & 0.0687(9) & 0.0618(7) & 0.1072(12) \\
\textbf{Monte Carlo} & 0.0263(11) & 0.0215(11) & 0.0378(11) & 0.0018(12) & 9.4474(12) & 0.1552(12) & 0.1107(12) & 0.0894(10) \\
\textbf{GARCH} & 0.0145(2) & 0.0166(9) & 0.0329(9) & 0.0009(7) & 3.9889(7) & 0.0533(7) & 0.0634(8) & 0.0772(7) \\
\textbf{E-GARCH} & 0.0153(4) & 0.0166(9) & 0.0327(8) & 0.001(8) & 4.549(9) & 0.062(8) & 0.0713(9) & 0.0782(8) \\
\textbf{CAViaR Symmetric} & 0.0177(8) & 0.0099(5) & 0.0303(5) & 0.0005(3) & 2.3903(3) & 0.0251(3) & 0.0484(5) & 0.0545(5) \\
\textbf{CAViaR Asymmetric} & 0.0139(1) & 0.0066(2) & 0.0255(1) & 0.0007(4) & 2.7576(5) & 0.0504(6) & 0.0426(3) & 0.0663(6) \\
\textbf{CAViaR Garch} & 0.0172(7) & 0.0099(4) & 0.0303(4) & 0.0004(2) & 1.9995(2) & 0.0185(2) & 0.0423(2) & 0.0508(4) \\
\textbf{CAViaR Adaptive} & 0.0225(10) & 0.0066(1) & 0.032(7) & 0.0003(1) & 1.2955(1) & 0.0135(1) & 0.0326(1) & 0.0316(2) \\
\textbf{Encoded VaR} & 0.017(6) & 0.0066(2) & 0.0268(2) & 0.0008(5) & 2.6656(4) & 0.044(5) & 0.0482(4) & 0.0461(3) \\

==> tabs/loss_table_SP_5.tex <==
% Table generated by Excel2LaTeX from sheet 'S&P'
\begin{table}[]
  \centering
  \caption{1-day 95\% VaR Losses(with their rank): S\&P500 portfolio}
    \begin{tabular}{lllllllll}
    \toprule
          & \textbf{Sener} & \textbf{Lopez} & \textbf{Sarma} & \textbf{Quadratic} & \textbf{Caporin 1} & \textbf{Caporin 2} & \textbf{Caporin 3} & \textbf{Quantile } \\
    \midrule
    \textbf{RiskMetrics} & 0.0608(8) & 0.0497(11) & 0.0607(11) & 0.0024(10) & 16.3142(9) & 0.2252(10) & 0.1653(10) & 0.0255(9) \\
    \textbf{Variance - Covariance} & 0.069(10) & 0.0447(6) & 0.0559(7) & 0.003(11) & 22.1855(11) & 0.3545(11) & 0.186(11) & 0.0282(11) \\
    \textbf{Historical} & 0.0752(11) & 0.0348(1) & 0.0503(2) & 0.0016(2) & 8.1736(1) & 0.1048(1) & 0.1275(2) & 0.0165(2) \\
    \textbf{Filtered Historical} & 0.0563(3) & 0.0464(8) & 0.0578(9) & 0.002(7) & 16.9587(10) & 0.2124(9) & 0.1503(7) & 0.0331(12) \\
    \textbf{Monte Carlo} & 0.0689(9) & 0.0447(6) & 0.0558(6) & 0.003(12) & 22.5353(12) & 0.3629(12) & 0.1877(12) & 0.0279(10) \\
    \textbf{GARCH} & 0.0567(5) & 0.0464(8) & 0.0574(8) & 0.002(6) & 13.7022(7) & 0.1674(7) & 0.1574(8) & 0.0197(6) \\
    \textbf{E-GARCH} & 0.06(7) & 0.0546(12) & 0.0654(12) & 0.0021(9) & 14.2935(8) & 0.1841(8) & 0.162(9) & 0.019(5) \\
    \textbf{CAViaR Symmetric} & 0.0563(3) & 0.043(5) & 0.0549(5) & 0.0019(5) & 11.266(5) & 0.1473(4) & 0.1437(5) & 0.0172(3) \\
    \textbf{CAViaR Asymmetric} & 0.0558(2) & 0.048(10) & 0.0598(10) & 0.0016(1) & 11.8779(6) & 0.153(5) & 0.1314(3) & 0.0237(8) \\
    \textbf{CAViaR Garch} & 0.0547(1) & 0.0364(2) & 0.0487(1) & 0.0017(3) & 10.2336(3) & 0.1291(2) & 0.133(4) & 0.0178(4) \\
    \textbf{CAViaR Adaptive} & 0.0764(12) & 0.0381(3) & 0.0528(4) & 0.002(8) & 10.7879(4) & 0.1565(6) & 0.1463(6) & 0.0226(7) \\
    \textbf{Encoded VaR} & 0.0568(6) & 0.0389(4) & 0.0516(3) & 0.0017(4) & 9.0391(2) & 0.1459(3) & 0.1176(1) & 0.0163(1) \\
    \bottomrule
    \end{tabular}%
  \label{tab:addlabel}%
\end{table}%


==> tabs/loss_table_TSX_5.tex <==

\begin{table}[]
  \centering
  \caption{1-day 95\% VaR Losses(with their rank): TSX portfolio}
    \begin{tabular}{lllllllll}
    \toprule
          & \textbf{Sener} & \textbf{Lopez} & \textbf{Sarma} & \textbf{Quadratic} & \textbf{Caporin 1} & \textbf{Caporin 2} & \textbf{Caporin 3} & \textbf{Quantile } \\
    \midrule
    \textbf{RiskMetrics} & 0.0456(8) & 0.0368(5) & 0.0467(5) & 0.0018(6) & 4.8563(3) & 0.1027(6) & 0.0658(3) & 0.0095(9) \\
    \textbf{Variance - Covariance} & 0.0514(10) & 0.0541(9) & 0.0642(10) & 0.0025(10) & 10.7461(9) & 0.2441(10) & 0.1026(9) & 0.0091(8) \\
    \textbf{Historical} & 0.045(5) & 0.0303(3) & 0.0416(3) & 0.0024(9) & 6.3303(5) & 0.2222(9) & 0.0685(4) & 0.0057(1) \\
    \textbf{Filtered Historical} & 0.0564(11) & 0.0606(11) & 0.0696(11) & 0.0021(7) & 11.1112(11) & 0.1565(7) & 0.1031(10) & 0.012(12) \\
    \textbf{Monte Carlo} & 0.051(9) & 0.0541(9) & 0.0641(9) & 0.0026(11) & 10.9752(10) & 0.2472(11) & 0.104(11) & 0.0086(6) \\
    \textbf{GARCH} & 0.045(5) & 0.0238(2) & 0.0345(2) & 0.0017(5) & 3.5205(2) & 0.0928(5) & 0.0534(2) & 0.0096(10) \\
    \textbf{E-GARCH} & 0.0441(4) & 0.0216(1) & 0.0325(1) & 0.0016(3) & 3.2467(1) & 0.0853(2) & 0.0509(1) & 0.0081(4) \\
    \textbf{CAViaR Symmetric} & 0.0438(3) & 0.0476(6) & 0.057(6) & 0.0015(1) & 6.1747(4) & 0.083(1) & 0.0685(5) & 0.0087(7) \\
    \textbf{CAViaR Asymmetric} & 0.038(1) & 0.0498(8) & 0.0593(8) & 0.0016(2) & 6.6781(7) & 0.087(3) & 0.0715(7) & 0.0083(5) \\
    \textbf{CAViaR Garch} & 0.045(5) & 0.0476(7) & 0.0572(7) & 0.0016(4) & 6.3629(6) & 0.0893(4) & 0.069(6) & 0.0114(11) \\
    \textbf{CAViaR Adaptive} & 0.0769(12) & 0.0714(12) & 0.0802(12) & 0.0031(12) & 19.3731(12) & 0.406(12) & 0.1449(12) & 0.0069(2) \\
    \textbf{Encoded VaR} & 0.0437(2) & 0.0306(4) & 0.0416(4) & 0.0024(8) & 7.2191(8) & 0.2081(8) & 0.0775(8) & 0.0078(3) \\

    \bottomrule
    \end{tabular}%
  \label{tab:addlabel}%
\end{table}%


==> tabs/temp1C.tex <==
\begin{table}[width=1.0\linewidth, cols=5, pos = h!]
  \centering
  \caption{Number of good and bads in each data set}
\begin{tabular*}{\tblwidth}{@{}LCCCCCCC@{}}
    \toprule
          & \multicolumn{2}{c}{German} & \multicolumn{2}{c}{Japan} & \multicolumn{2}{c}{Australia} \\
          \midrule
          & train & test  & train & test  & train & test \\
    \midrule
    good  & 458   & 242   & 206   & 91    & 206   & 101 \\
    bad   & 458   & 92    & 234   & 130   & 254   & 129 \\
    \bottomrule
    
    \end{tabular*}%
    \label{tab:train_test}%
\end{table}%

==> tabs/temp2C.tex <==
\begin{table*}[width=2.0\linewidth, cols=5, pos = h!]
  \centering
  \caption{Comparison of Our Model's accuracy to SVM and LR}
\begin{tabular*}{\tblwidth}{@{}LCCCCCCC@{}}

    \toprule
          & \multicolumn{2}{c}{German} & \multicolumn{2}{c}{Japan} & \multicolumn{2}{c}{Australia} \\
          & \multicolumn{1}{c}{train} & \multicolumn{1}{c}{test} & \multicolumn{1}{c}{train} & \multicolumn{1}{c}{test} & \multicolumn{1}{c}{train} & \multicolumn{1}{c}{test} \\
    \midrule
    accuracy & 74.23\% & 72.15\% & 84.31\% & 84.16\% & 82.39\% & 80.00\% \\
    SVM   & 54.80\% & 66.76\% & 65.68\% & 68.77\% & 66.52\% & 66.08\% \\
    LR    & 82.31\% & 73.95\% & 82.50\% & 84.10\% & 84.56\% & 81.73\% \\
    \bottomrule
    \end{tabular*}%
    \label{tab:accuracies}%
\end{table*}%
